Nonlinearities in Macroeconomic Tail Risk through the Lens of Big Data Quantile Regressions

Modeling and predicting extreme movements in GDP is notoriously difficult and the selection of appropriate covariates and/or possible forms of nonlinearities are key in obtaining precise forecasts. In this paper, our focus is on using large datasets in quantile regression models to forecast the conditional distribution of US GDP growth. To capture possible non-linearities, we include several nonlinear specifications. The resulting models will be huge dimensional and we thus rely on a set of shrinkage priors. Since Markov Chain Monte Carlo estimation becomes slow in these dimensions, we rely on fast variational Bayes approximations to the posterior distribution of the coefficients and the latent states. We find that our proposed set of models produces precise forecasts. These gains are especially pronounced in the tails. Using Gaussian processes to approximate the nonlinear component of the model further improves the good performance, in particular in the right tail.

==> 00_praembel.tex <==
\usepackage[a4paper, textwidth=14.5cm, left=2.5 cm, right=2.5 cm, top=2cm,bottom=3cm]{geometry}
% Packages
\usepackage[american]{babel}        % Spracheinstellung
\usepackage[ansinew, utf8]{inputenc}         % Umlaute
\usepackage{setspace}   % Setzte den Zeilanabstand auf 1/1/2
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{dsfont}
%\usepackage{dstroke}
\usepackage{upgreek}
\usepackage{eqnarray}
\usepackage{longtable}
\usepackage{pdflscape}
\usepackage{epstopdf}
\usepackage[T1]{fontenc}
\usepackage{pdflscape}
\usepackage[table,xcdraw]{xcolor}
\usepackage{framed}
\usepackage{subfigure}
\usepackage{bbding}
\usepackage{caption}
\captionsetup[table]{position=bottom}
% \usepackage{subcaption}
% \onehalfspacing
\doublespacing

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Section Title in header %%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{fancyhdr}
%\pagestyle{fancy}
%\fancyhf{}
%\fancyhead[L]{\leftmark}
%\fancyfoot[C]{\thepage}
%\renewcommand{\sectionmark}[1]{\markboth{#1}{}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Abk?rzungsverzeichnis %%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[printonlyused]{acronym}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% L?sst Grafiken sch?ner flie?en %%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{float}                          % L?sst Grafiken sch?ner flie?en

%bib
%\usepackage[square,numbers,sort&compress]{natbib}
\usepackage[authoryear]{natbib}
\bibliographystyle{apalike} 


%%%%% floatplacement (let pictures float in a better way)
\renewcommand{\topfraction}{0.9}        % max fraction of floats at top
    \renewcommand{\bottomfraction}{0.5} % max fraction of floats at bottom
    % Parameters for TEXT pages (not float pages):
    \setcounter{topnumber}{2}
    \setcounter{bottomnumber}{2}
    \setcounter{totalnumber}{4}     % 2 may work better
    \setcounter{dbltopnumber}{2}    % for 2-column pages
    \renewcommand{\dbltopfraction}{0.9} % fit big float above 2-col. text
    \renewcommand{\textfraction}{0.07}  % allow minimal text w. figs
    % Parameters for FLOAT pages (not text pages):
    \renewcommand{\floatpagefraction}{0.7}      % require fuller float pages
    % N.B.: floatpagefraction MUST be less than topfraction !!
%%%%%



\usepackage{graphicx}
%\usepackage[margin=1.5em,textfont={small}]{subfig}

% Caption, Subfig, Tables, etc. + settings
% positioning of figures, etc.
%\usepackage{float}  % use float instead of floatrow if you work with knitr (positioning of figurers within chunks needs float)
\floatstyle{plaintop}
\restylefloat{table}
% numbered annotation inside the figure- and table-environment \caption[short description]{long description}
\usepackage[width=0.8\linewidth,
            textfont={small},
            labelfont={small, bf},
            format=plain,
            justification=justified,
            aboveskip=4pt,
            parskip=0pt]
            {caption}
\usepackage[innercaption]{sidecap}
\renewcommand{\sidecaptionsep}{0.02\linewidth}
%more
\usepackage{theorem,ifthen,exscale}
\usepackage{tabularx,dcolumn,booktabs}
\usepackage{multirow}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Operatoren commands %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\rmd}{\text{d}}
\DeclareMathOperator{\vek}{vec}
\DeclareMathOperator{\pr}{P}
\DeclareMathOperator{\N}{N}
\DeclareMathOperator{\IW}{IW}
\DeclareMathOperator{\tr}{tr}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% R?mische Zahlen %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\RM}[1]{\MakeUppercase{\romannumeral #1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Define new citecommand %%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{xifthen}
\newcommand{\zito}[2][]{\citeauthor{#2} (\citeyear{#2}\ifthenelse{\isempty{#1}}{}{, #1})}
\newcommand{\zitt}[2][]{(\citeauthor{#2}, \citeyear{#2}\ifthenelse{\isempty{#1}}{}{, #1})}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Define Defintion setting %%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{defn}{Definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Define new citecommand %%%%%%%%%%%%%%%%%%%%%%%%%%
% Hyperlinks + settings "load hyperref as the last package"
% http://norwied.wordpress.com/2012/07/10/how-to-break-long-urls-in-bibtex/
\usepackage{url}
\usepackage{breakurl}
\def\UrlBreaks{\do\/\do-\do\_}  % Break signs: '\', '-', '_'
\usepackage[hyperfootnotes=false]{hyperref}  % no footnotelinks;solves:warning: name(Hfootnote.xx) ...
    \hypersetup{
    bookmarksnumbered,                    % bookmarks
    unicode=false,                        % non-Latin characters inAcrobat?s bookmarks
    pdftoolbar=true,                      % show Acrobat?s toolbar?
    pdfmenubar=true,                      % show Acrobat?s menu?
    pdffitwindow=false,                   % window fit to page when opened
    pdfstartview={FitH},                  % fits the width of the pageto the window
    pdftitle={My title},                  % title
    pdfauthor={Author},                   % author
    pdfsubject={Subject},                 % subject of the document
    pdfcreator={Creator},                 % creator of the document
    pdfproducer={Producer},               % producer of the document
    pdfkeywords={keyword1} {key2} {key3}, % list of keywords
    pdfnewwindow=true,                    % links in new window
    colorlinks=true,                      % false: boxed links; true:colored links
    linkcolor=black,                      % color of internal links
    citecolor=black,                      % color of links to bibliography
    filecolor=black,                      % color of file links
    urlcolor=[RGB]{51,51,51}              % color of external links
    }
%
%\linespread{2}

\usepackage{titling}
%(\textit{Preliminary, do not cite do not publish})
\title{Responses to comments on: Nonlinearities in Macroeconomic Tail Risk through the Lens of
Big Data Quantile Regressions
\\}
 
